Survey on video anomaly detection in dynamic scenes with moving cameras

The increasing popularity of compact and inexpensive cameras, e.g.~dash cameras, body cameras, and cameras equipped on robots, has sparked a growing interest in detecting anomalies within dynamic scenes recorded by moving cameras. However, existing reviews primarily concentrate on Video Anomaly Detection (VAD) methods assuming static cameras. The VAD literature with moving cameras remains fragmented, lacking comprehensive reviews to date. To address this gap, we endeavor to present the first comprehensive survey on Moving Camera Video Anomaly Detection (MC-VAD). We delve into the research papers related to MC-VAD, critically assessing their limitations and highlighting associated challenges. Our exploration encompasses three application domains: security, urban transportation, and marine environments, which in turn cover six specific tasks. We compile an extensive list of 25 publicly-available datasets spanning four distinct environments: underwater, water surface, ground, and aerial. We summarize the types of anomalies these datasets correspond to or contain, and present five main categories of approaches for detecting such anomalies. Lastly, we identify future research directions and discuss novel contributions that could advance the field of MC-VAD. With this survey, we aim to offer a valuable reference for researchers and practitioners striving to develop and advance state-of-the-art MC-VAD methods.

==> sections/related_survey.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Related surveys}\label{sec:related_surveys}

We mainly cover the recent surveys on VAD~\citep{deepvad2021,surveyAD,surveypami,AIreview22,survey2021multimedia}, relevant topics including abnormal human behaviors~\citep{popoola2012video,Poiesi2015,surveyHAR}, and hazard detection in autonomous driving~\citep{10038646}. 

Among the surveys on VAD, some serve as a summary of research progress in VAD~\citep{deepvad2021} while others focus on either the method categorization~\citep{surveyAD,surveypami,AIreview22} or the datasets organization~\citep{survey2021multimedia}.
\cite{deepvad2021} provide a high-level review on deep video anomaly detection in terms of the challenges and potential opportunities in fields such as intelligent transportation, digital education, smart home, public health, and digital twins. 
Although intelligent transportation is a primary application area of MC-VAD, this survey lacks details in aspects including datasets, approaches, and challenges for each practical application.

There also exist surveys that cast their focus on more specific aspects among the vast VAD literature.
For example, \cite{surveyAD} offer a review of the deep learning methods that address VAD with a comprehensive taxonomy and a detailed discussion in terms of their key intuitions, objective functions, underlying assumptions, advantages, and disadvantages. 
A similar survey by \cite{AIreview22} covers more recent deep-learning-based methods on VAD.~\cite{surveypami} identify the differences between the attributes of anomalies in the single-scene and multi-scene setup, and focus on the research progresses on VAD with videos featuring a single scene. They categorize approaches and provide various problem formulations and a comprehensive comparison of the accuracy of many algorithms on standard test sets. 
\cite{survey2021multimedia} focus on multimedia datasets for the study of VAD. 
They divide these datasets into video anomaly datasets, audio anomaly datasets, and audio-visual anomaly datasets.
For video anomaly datasets, the authors list more than 30 publicly available video datasets used for anomaly detection from 2007 to 2020. 
While the list is comprehensive for the study of SC-VAD, there is only one dataset that is related to moving cameras in their survey.
In general, the above-mentioned surveys primarily focus on SC-VAD and pay little attention to moving cameras, not reflecting the differences and challenges of MC-VAD.

We believe that human activity recognition (HAR) or human abnormal behavior detection is relevant to the application of VAD as human activity is one of the main causes of video anomalies.~\cite{popoola2012video} focus on video-based abnormal human behavior recognition. 
This survey starts with human motion analysis and then discusses the contextual characteristics of anomalies, scene modeling, as well as behavior abstraction and representation, providing a comprehensive survey of human VAD from the bottom up. 
They highlight that the definition of anomaly can have some degree of ambiguity within a domain of application, which is very important to MC-VAD. ~\cite{Poiesi2015} survey methods for the analysis of human interactions in public places, which in turn can be used to detect situations of panic.~\cite{surveyHAR} discuss each step of the complete process of HAR technology and discussed the feature extraction, coding technology, and action analysis technology, providing a basis for human detection in VAD. 
However, these surveys are not primarily concerned with moving camera video anomaly detection. 
Additionally, they only study people, while the objects concerning anomalies in MC-VAD can often be non-human objects such as cars and obstacles.

Lastly,~\cite{10038646} focuses on graph-based hazardous event detection in autonomous driving scenarios. 
They provide a comprehensive and detailed classification and definition of hazardous event categories within the autonomous driving scenario. 
An overview of graph-based methods thoroughly summarizes the corresponding datasets and evaluation metrics. However, the analysis does not cover anomaly detection with moving cameras in other application scenarios.

To the best of our knowledge, ours is the first and most comprehensive survey on MC-VAD. 
We begin by introducing the concept of MC-VAD, which builds upon the fundamental principles of VAD, but incorporates new challenges posed by the camera motion.
Our survey provides an extensive overview of research progress in MC-VAD from 2012 to 2022, covering three broad application areas with an organized summary of 24 datasets collected from moving cameras for the study of MC-VAD. 
We also organize these methods into five categories for addressing MC-VAD with a discussion of their respective advantages and limitations.

Tab.~\ref{tab0} summarizes several noteworthy surveys for MC-VAD and their applications.

\input{tables/related_survey}








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
